The hybrid approach -- Convolutional Neural Networks and Expectation Maximization Algorithm -- for Tomographic Reconstruction of Hyperspectral Images

We present a simple but novel hybrid approach to hyperspectral data cube reconstruction from computed tomography imaging spectrometry (CTIS) images that sequentially combines neural networks and the iterative Expectation Maximization (EM) algorithm. We train and test the ability of the method to reconstruct data cubes of $100\times100\times25$ and $100\times100\times100$ voxels, corresponding to 25 and 100 spectral channels, from simulated CTIS images generated by our CTIS simulator. The hybrid approach utilizes the inherent strength of the Convolutional Neural Network (CNN) with regard to noise and its ability to yield consistent reconstructions and make use of the EM algorithm's ability to generalize to spectral images of any object without training. The hybrid approach achieves better performance than both the CNNs and EM alone for seen (included in CNN training) and unseen (excluded from CNN training) cubes for both the 25- and 100-channel cases. For the 25 spectral channels, the improvements from CNN to the hybrid model (CNN + EM) in terms of the mean-squared errors are between 14-26%. For 100 spectral channels, the improvements between 19-40% are attained with the largest improvement of 40% for the unseen data, to which the CNNs are not exposed during the training.

==> supplement_part.tex <==
\makeatletter
\pagebreak


\setcounter{section}{0}
\setcounter{equation}{0}
\setcounter{figure}{0}
\setcounter{table}{0}
\setcounter{page}{1}
\renewcommand{\thefigure}{S\arabic{figure}}
\renewcommand{\thesection}{S\arabic{section}}

%\title{Supplemental material}
%\maketitle
\begin{center}
	\textbf{\large Supplemental material}\\[.2cm]
	Mads Juul Ahleb{\ae}k,$^{1}$ Mads Svanborg Peters,$^{2,3}$, Wei-Chih Huang$^1$, Mads Toudal Frandsen,$^{1}$, Ren\'e Lynge Eriksen$^{3}$ and Bjarke J{\o}rgensen$^{2}$ \\[.1cm]
	{\itshape ${}^1$\small{CP$^3$-Origins, Department of Physics, Chemistry and Pharmacy, \\ University of Southern Denmark, Denmark}\\
		${}^2$\small{Newtec Engineering A/S, 5230 Odense, Denmark}\\
		${}^3$\small{Mads Clausen Institute, University of Southern Denmark, Denmark}\\}
	%(Dated: \today)\\[1cm]
\end{center}

%\author{\small{Mads Juul Ahleb{\ae}k}}
%\email{maahl17@student.sdu.dk}
%\affiliation{\small{CP$^3$-Origins, Department of Physics, Chemistry and Pharmacy, University of Southern Denmark, Denmark}}

%\author{\small{Mads Svanborg Peters}}
%\email{mape@newtec.dk}
%\affiliation{\small{Newtec Engineering A/S, 5230 Odense, Denmark}}
%\affiliation{\small{Mads Clausen Institute, University of Southern Denmark, Denmark}}

%\author{\small{Wei-Chih Huang}}
%\email{huang@cp3.sdu.dk}
%\affiliation{\small{CP$^3$-Origins, Department of Physics, Chemistry and Pharmacy, University of Southern Denmark, Denmark}}


%\author{\small{Mads Toudal Frandsen}}
%\email{frandsen@cp3.sdu.dk}
%\affiliation{\small{CP$^3$-Origins, Department of Physics, Chemistry and Pharmacy, University of Southern Denmark, Denmark}}

%\author{\small{Ren\'e Lynge Eriksen}}
%\email{rle@mci.sdu.dk}
%\affiliation{\small{Mads Clausen Institute, University of Southern Denmark, Denmark}}

%\author{\small{Bjarke J{\o}rgensen}}
%\email{bjarke@newtec.dk}
%\affiliation{\small{Newtec Engineering A/S, 5230 Odense, Denmark}}


\section{Introduction}\label{sec:S1}
This supplemental material accompanies the main paper and details the computed tomography imaging spectrometer (CTIS) simulator as well as the measurement of the parameters used in the simulator. Additionally, RGB visualizations of all the hyperspectral images captured with our VIS-NIR laboratory pushbroom system are shown. A selection of the reconstructed hyperspectral images for both the 25- and 100-channel cases are also compared through RGB visualizations. 
\section{Computed tomography imaging spectrometer simulator}\label{sec:simulator}
The CTIS simulator introduced in our work is an updated version of the simulator used in our previous work \cite{huang2022application}, and is used to create input CTIS images for our network. This updated simulator includes zero mean white Gaussian noise, a point spread function (PSF) and spectral sensitivity corrections due to the illuminant and the diffractive optic element (DOE). Thus, the simulator requires the following inputs; \texttt{x}, \texttt{y}, \texttt{z}, \texttt{b1}, \texttt{b2}, \texttt{shift}, \texttt{allOrders}, \texttt{diff\_sens}, \texttt{illum}, \texttt{sigma\_psf} and \texttt{noise}. The first seven inputs determine the geometry of simulated CTIS image while the latter three inputs determine the optical parameters.

Fig.~\ref{fig:input_a} shows an overview of how the geometric inputs correlate to the simulated CTIS image: \texttt{x}, \texttt{y}, and \texttt{z} denote the two spatial and one spectral dimension of the input respectively, i.e. the zeroth order size is defined by \texttt{x}$\times$\texttt{y} and \texttt{z} denotes the number of spectral channels. \texttt{b1} and \texttt{b2} determine the number of pixels between the zeroth- and first orders and the first orders and the outer border of the image, respectively. \texttt{b2} is usually set to zero, but provided for generalizability. The \texttt{shift} input determines the pixel-shift between consecutive spectral channels in the first order diffraction spots. It should be mentioned, that the user is responsible for setting the inputs to the correct values to match the true CTIS system, i.e. \texttt{b1}, \texttt{b2} and \texttt{shift} are not calculated in the simulator based on the wavelengths of the spectral channels. The \texttt{allOrders} input is a boolean parameter, which simulates all eight surrounding first order diffraction spots if set to true and only the four (no skew orders) first order diffraction spots if set to false. 
\begin{figure}[htp]
	\begin{center}
		\subfloat[]{\includegraphics[width = 0.49\textwidth]{fig/overview_input}\label{fig:input_a}} \hfill 
		\subfloat[]{\includegraphics[width = 0.469\textwidth]{fig/ctis-g-example_noaxis.pdf}\label{fig:input_b}}
	\end{center}
	\caption{(a) Visual overview of the correspondence between the geometric inputs of the CTIS simulator and the simulated CTIS image for inputs \texttt{x}, \texttt{y}, \texttt{z}, \texttt{b1} = 5, \texttt{b2} = 0, \texttt{shift} = 2, \texttt{allOrders} = true, and without \texttt{sigma\_psf}, \texttt{diff\_sens}, \texttt{illum} or \texttt{noise}. (b) Simulated CTIS image for \texttt{x},\texttt{y} = 100, \texttt{z} = 25, \texttt{b1} = 27, \texttt{b2} = 0, \texttt{shift} = 2, \texttt{allOrders} = true, \texttt{sigma\_psf} = 1.04 and \texttt{noise} = 0.44. \texttt{diff\_sens} and \texttt{illum} are set to the values defined in Sec.~\ref{app:sensitivity}}
	\label{fig:input_overview}
\end{figure} 

The optical parameters of the CTIS system is defined by the \texttt{diff\_sens}, the \texttt{illum} and the applied \texttt{noise}. Additionally, the point-spread-function (PSF), \texttt{sigma\_psf}, is set within the simulator, but is not available to the user as an input. The measurement of the PSF for the true CTIS system is detailed in Sec.~\ref{app:psf}. The \texttt{diff\_sens} describes the wavelength- and diffraction order dependent sensitivity and must be a matrix of dimensions $\# \text{ orders} \times$\texttt{z}, i.e. in the case of \texttt{allOrders = true}, $9\times$\texttt{z}. The acquisition of the diffraction sensitivity is described in Sec.~\ref{app:sensitivity}. The illuminant used in the simulator is a standard halogen-tungsten lamp, which is used for the acquisition of true CTIS images. The illumination input is a vector of size $1\times z$, which contains the spectrum of the illuminant measured with an intensity calibrated Avaspec 2048x14 spectrometer operating in the 200-720~nm range. The spectrometer was calibrated using a radiometrically calibrated light source (HL-3P-CAL) from Ocean Insights.

 Fig.~\ref{fig:input_b} shows a simulated $450\times450$~pixels CTIS image of a $100\times100\times25$ white cube, i.e. all voxels are set to 1, with \texttt{b1} = 27, \texttt{b2} = 0, \texttt{shift} = 2, \texttt{allOrders} = true, \texttt{sigma\_psf} = $\sigma=1.04$~pixels and \texttt{noise} = 0.44. The diffraction sensitivity and illumination is set to the values defined in Sec.~\ref{app:sensitivity}.
 
 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}[htp]
	\begin{center}
		\includegraphics[width = \textwidth]{fig/slanted_edge.pdf}
	\end{center}
	\caption{(a) CTIS image of a slanted razorblade back illuminated by tungsten halogen lamps for point spread function (PSF) estimation. (b) zeroth order of CTIS image with $250\times40$ pixels blue rectangle used to estimate the (c) edge spread function (ESF) (mean across 250 pixels) and (d) line spread function (LSF) (derivative of ESF). The standard deviation of the LSF is estimated from a Gaussian fit, and (e) depicts the estimated symmetric PSF.}
	\label{fig:slanted_edge}
\end{figure} 
\section{Measurements of point spread function} \label{app:psf} 
The PSF of the CTIS system is determined using the slanted-edge method~\cite{estribeau_fast_2004}, where a sharp, slanted image is imaged and the PSF is estimated from the transition of the edge. In practice, a back illuminated razorblade is imaged by the CTIS camera (Fig.~\ref{fig:slanted_edge}\red{a}), and the edge spread function (ESF) (Fig.~\ref{fig:slanted_edge}\red{c}) is calculated as the mean profile across 250~pixels (blue rectangle) over the transition in the zeroth order (Fig.~\ref{fig:slanted_edge}\red{b}). The line spread function (LSF) is depicted in Fig.~\ref{fig:slanted_edge}\red{d}, and it is calculated as the derivative of the ESF, which is equivalent to a 2D slice of the PSF. Thus, assuming a spatially symmetric PSF, the LSF is an approximate estimate of the PSF. The standard deviation of the LSF (and PSF) is determined to be 1.04 pixels based on a Gaussian fit with $R^2=0.98$. The effect of the PSF on a single pixel is visualized in Fig.~\ref{fig:slanted_edge}\red{e} for a standard deviation of 1.04, which is the value used in the simulator.


\section{Measurement of diffraction sensitivity}\label{app:sensitivity}
The diffraction sensitivity of the CTIS system is measured using a monochromator (Newport mini, model: 78027) equipped with a halogen lamp (Tungsten Halogen Light Source, model:
78043), which is calibrated with an intensity calibrated Avaspec 2048x14 spectrometer. The spectrometer is calibrated using a radiometrically calibrated light source (HL-3P-CAL) from Ocean Insights. Since the measurements are conducted with the whole CTIS system, both the diffraction efficiency of the DOE, the transmission of the optical system, the CMOS image sensor response and optical aberrations are intrinsically a part of the acquired images. Thus, the measured diffraction sensitivity estimates the combined contribution from all these contributions. The monochromator output is centered in the zeroth order of the CTIS image, and CTIS images and corresponding dark-frame images are captured for wavelengths ranging from 400-750 nm with 25 nm steps. For each wavelength, the exposure time of the CTIS is set to maximize the dynamic range of the image sensor, and the dark frame is captured at the same exposure. Fig.~\ref{fig:diff_sens}\red{a} shows the superimposed CTIS images of the monochromator for 400-750 nm.  
\begin{figure}[htp]
	\begin{center}
		\includegraphics[width = \textwidth]{fig/diff_sensitivity2.pdf}
	\end{center}
	\caption{(a) superimposed image consisting of monochromator images for 400-750 nm with 25 nm steps. (b) Normalized monochromator photon count measured with a calibrated Avaspec 2048x14 spectrometer, and correction factors corresponding to the area under the curve. (c) calculated diffraction sensitivity $S(\lambda,s)$ for the wavelength range 400-750 nm and the 9 diffraction order spots.}
	\label{fig:diff_sens}
\end{figure} 
To determine the diffraction sensitivity $S(\lambda,s)$ from the acquired images, the dark frame is subtracted from the CTIS image, and the total photon count $PC(\lambda,s)$ for each diffraction spot (zeroth- and surrounding first orders) is divided with the product of the exposure time $t(\lambda)$ in \textmu s, the camera gain $G(\lambda)$ (set to 1 for all images) and the wavelength correction factor $C(\lambda)$ from the spectrometer:
\begin{align}
	S(\lambda,s) = \frac{PC(\lambda,s)}{t(\lambda) \cdot G(\lambda) \cdot C(\lambda)},
\end{align}
where $\lambda$ and $s$ denote the wavelength in nm and $s$ the diffraction spot, respectively. The monochromator output (Fig.~\ref{fig:diff_sens}\red{b}) is used to determine the correction factors $C(\lambda)$, which indicate the relative intensity of the monochromator output (area in blue under the curve). The total photon count of the respective diffraction spots $PC(\lambda,s)$ is determined from the acquired CTIS images as the total volume of each spot. Fig.~\ref{fig:diff_sens}\red{c} shows the calculated diffraction sensitivity $S(\lambda,s)$, where the indices ($i$, $j$) of the diffraction spots indicate (rows, columns). The DOE is designed to achieve a symmetric diffraction efficiency in the first orders while minimizing the zeroth order. The diffraction sensitivity of the zeroth order (0,0) is smallest for the lower wavelengths before increasing towards 700 nm, while the first order diffraction sensitivities all follow the same parabolic shape. However, the right-diagonal first orders \{(-1,1) and (1,1)\} have significantly lower diffraction sensitivity across the entire wavelength range. It should be noted, that since $S(\lambda,s)$ is only measured for 15 different wavelengths from 400-750 nm, the sensitivities are interpolated for the 25 and 100 channels used in this work. 


 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\section{Measurement of halogen lamp illumination}\label{app:illumination}
The intensity calibrated Avaspec 2048x14 spectrometer is used to measure the output of an industrial halogen lamp used as illumination for the acquisition of CTIS images. Fig.~\ref{fig:illum} shows the measured spectrum of the halogen lamp and a fitted black body with a temperature of $T = 2952$~K\degree, which is consistent with standard $T = 3000$~K\degree~halogen lamps . 
\begin{figure}[htp]
	\begin{center}´
		\includegraphics[width = \textwidth]{fig/illumination.pdf}
	\end{center}
	\caption{Measured spectrum of the industrial $3000$~K\degree~halogen lamps used as illumination for CTIS images and a fitted black body with a temperature of $T = 2952$~K\degree.}
	\label{fig:illum}
\end{figure} 

\section{RGB reconstruction of pushbroom hyperspectral cubes}\label{app:RGB_cubes}
Fig.~\ref{fig:supp_rgb_1}-\ref{fig:supp_rgb_4} shows RGB reconstructions of the 178 hyperspectral images captured with the VIS-NIR pushbroom system, which were used to generate data sets of CTIS images for the networks. The RGB images are generated by combining three spectral channels at 470~nm (blue), 549~nm (green) and 650~nm (red). 
\begin{figure}[h]
	\begin{center}
		\includegraphics[width = \textwidth]{fig/supplem/pushbroom_rgb_1names_topbar}\par\bigskip
		\includegraphics[width = \textwidth]{fig/supplem/pushbroom_rgb_2names_topbar}
	\end{center}
	\caption{\textbf{(1)} RGB reconstructions of hyperspectral images captured with the pushbroom system and used in the training of the neural networks.}
	\label{fig:supp_rgb_1}
\end{figure} 

\begin{figure}[h]
	\begin{center}
		\includegraphics[width = \textwidth]{fig/supplem/pushbroom_rgb_3names_topbar}\par\bigskip
		\includegraphics[width = \textwidth]{fig/supplem/pushbroom_rgb_4names_topbar}
	\end{center}
	\caption{\textbf{(2)} RGB reconstructions of hyperspectral images captured with the pushbroom system and used in the training of the neural networks.}
	\label{fig:supp_rgb_2}
\end{figure} 

\begin{figure}[h]
	\begin{center}
		\includegraphics[width = \textwidth]{fig/supplem/pushbroom_rgb_5names_topbar}\par\bigskip
		\includegraphics[width = \textwidth]{fig/supplem/pushbroom_rgb_6names_topbar}
	\end{center}
	\caption{\textbf{(3)} RGB reconstructions of hyperspectral images captured with the pushbroom system and used in the training of the neural networks.}
	\label{fig:supp_rgb_3}
\end{figure} 

\begin{figure}[h]
	\begin{center}
		\includegraphics[width = \textwidth]{fig/supplem/pushbroom_rgb_7names_topbar}\par\bigskip
		\includegraphics[width = \textwidth]{fig/supplem/pushbroom_rgb_8names_topbar}
	\end{center}
	\caption{\textbf{(4)} RGB reconstructions of hyperspectral images captured with the pushbroom system and used in the training of the neural networks.}
	\label{fig:supp_rgb_4}
\end{figure} 

\clearpage
\section{Comparison of RGB reconstructions for reconstructed hyperspectral cubes - 25 channels}\label{sec:suppl_25}
Fig.~\ref{fig:recon_rgb_1}-\ref{fig:recon_rgb_3} show comparisons of the ground truth (GT) RGB visualization with the reconstructed RGB images for EM(20 iterations), CNN, CNN-EM(10 iterations), EM(10 iterations)-CNN, UNet and UNet-EM(10 iterations) for various hyperspectral images. The RGB images are generated by combining the 7th, 9th and 13th channel. Fig.~\ref{fig:recon_rgb_1} and \ref{fig:recon_rgb_2} contain seen cubes used in the training, while Fig.~\ref{fig:recon_rgb_3} contains unseen cubes.

\begin{figure}[h]
	\begin{center}
		\includegraphics[width = \textwidth]{fig/supplem/100x100x25_RGB_4}
	\end{center}
	\caption{RGB comparison of reconstructed hyperspectral cubes (seen) for 25 channels. RGB images are generated from spectral channel 7, 9 and 13.}
	\label{fig:recon_rgb_1}
\end{figure} 


\begin{figure}[h]
	\begin{center}
		\includegraphics[width = \textwidth]{fig/supplem/100x100x25_RGB_6}
	\end{center}
	\caption{RGB comparison of reconstructed hyperspectral cubes (seen) for 25 channels. RGB images are generated from spectral channel 7, 9 and 13.}
	\label{fig:recon_rgb_2}
\end{figure} 

\begin{figure}[h]
	\begin{center}
		\includegraphics[width = \textwidth]{fig/supplem/100x100x25_RGB_1_unseen}
	\end{center}
	\caption{RGB comparison of reconstructed hyperspectral cubes (unseen) for 25 channels. RGB images are generated from spectral channel 7, 9 and 13.}
	\label{fig:recon_rgb_3}
\end{figure} 

\newpage
\section{Comparison of RGB reconstructions for reconstructed hyperspectral cubes - 100 channels}\label{sec:suppl_100}
Fig.~\ref{fig:recon_100_rgb_1}-\ref{fig:recon_100_rgb_3} show comparisons of the ground truth (GT) RGB visualization with the reconstructed RGB images for EM(20 iterations), UNet and UNet-EM(10 iterations) for various hyperspectral images. The RGB images are generated by combining the 14th, 29th and 48th channel. Fig.~\ref{fig:recon_100_rgb_1} and \ref{fig:recon_100_rgb_2} contain seen cubes used in the training, while Fig.~\ref{fig:recon_100_rgb_3} contains unseen cubes.
\begin{figure}[h]
	\begin{center}
		\includegraphics[width = .65\textwidth]{fig/supplem/100x100x100_RGB_5_seen}
	\end{center}
	\caption{RGB comparison of reconstructed hyperspectral cubes (seen) for 100 channels. RGB images are generated from spectral channel 14, 29 and 48.}
	\label{fig:recon_100_rgb_1}
\end{figure} 

\begin{figure}[h]
	\begin{center}
		\includegraphics[width = .65\textwidth]{fig/supplem/100x100x100_RGB_6_seen}
	\end{center}
	\caption{RGB comparison of reconstructed hyperspectral cubes (seen) for 100 channels. RGB images are generated from spectral channel 14, 29 and 48.}
	\label{fig:recon_100_rgb_2}
\end{figure} 

\begin{figure}[h]
	\begin{center}
		\includegraphics[width = .65\textwidth]{fig/supplem/100x100x100_RGB_1_seen}
	\end{center}
	\caption{RGB comparison of reconstructed hyperspectral cubes (unseen) for 100 channels. RGB images are generated from spectral channel 14, 29 and 48.}
	\label{fig:recon_100_rgb_3}
\end{figure} 



%\newpage
%\bibliography{ref_suppl}





